Physics-Informed Heterogeneous Graph Neural Networks for DC Blocker Placement

The threat of geomagnetic disturbances (GMDs) to the reliable operation of the bulk energy system has spurred the development of effective strategies for mitigating their impacts. One such approach involves placing transformer neutral blocking devices, which interrupt the path of geomagnetically induced currents (GICs) to limit their impact. The high cost of these devices and the sparsity of transformers that experience high GICs during GMD events, however, calls for a sparse placement strategy that involves high computational cost. To address this challenge, we developed a physics-informed heterogeneous graph neural network (PIHGNN) for solving the graph-based dc-blocker placement problem. Our approach combines a heterogeneous graph neural network (HGNN) with a physics-informed neural network (PINN) to capture the diverse types of nodes and edges in ac/dc networks and incorporates the physical laws of the power grid. We train the PIHGNN model using a surrogate power flow model and validate it using case studies. Results demonstrate that PIHGNN can effectively and efficiently support the deployment of GIC dc-current blockers, ensuring the continued supply of electricity to meet societal demands. Our approach has the potential to contribute to the development of more reliable and resilient power grids capable of withstanding the growing threat that GMDs pose.

==> Definitions.tex <==
\ProvidesPackage{Definitions}
% math fonts
\RequirePackage{amsmath}    % mathbf, mathrm, mathcal, mathsf, mathtt, mathit
\RequirePackage{amsfonts}   % mathbb, mathfrek
\RequirePackage{amssymb}
\RequirePackage{dsfont}     % mathds
\RequirePackage{amsthm}
\RequirePackage{mathrsfs}   % mathscr

% \RequirePackage{eucal} % mathscr
% \RequirePackage{mathrsfs}
% \RequirePackage{latexsym}
% \RequirePackage{bm}
% \RequirePackage{xspace}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

% mathbf
\newcommand{\Abf}{\mathbf{A}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\Cbf}{\mathbf{C}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\Ebf}{\mathbf{E}}
\newcommand{\Fbf}{\mathbf{F}}
\newcommand{\Gbf}{\mathbf{G}}
\newcommand{\Hbf}{\mathbf{H}}
\newcommand{\Ibf}{\mathbf{I}}
\newcommand{\Jbf}{\mathbf{J}}
\newcommand{\Kbf}{\mathbf{K}}
\newcommand{\Lbf}{\mathbf{L}}
\newcommand{\Mbf}{\mathbf{M}}
\newcommand{\Nbf}{\mathbf{N}}
\newcommand{\Obf}{\mathbf{O}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Qbf}{\mathbf{Q}}
\newcommand{\Rbf}{\mathbf{R}}
\newcommand{\Sbf}{\mathbf{S}}
\newcommand{\Tbf}{\mathbf{T}}
\newcommand{\Ubf}{\mathbf{U}}
\newcommand{\Vbf}{\mathbf{V}}
\newcommand{\Wbf}{\mathbf{W}}
\newcommand{\Xbf}{\mathbf{X}}
\newcommand{\Ybf}{\mathbf{Y}}
\newcommand{\Zbf}{\mathbf{Z}}

% \newcommand{\Ab}{\mathbf{A}}
% \newcommand{\Bb}{\mathbf{B}}
% \newcommand{\Cb}{\mathbf{C}}
% \newcommand{\Db}{\mathbf{D}}
% \newcommand{\Eb}{\mathbf{E}}
% \newcommand{\Fb}{\mathbf{F}}
% \newcommand{\Gb}{\mathbf{G}}
% \newcommand{\Hb}{\mathbf{H}}
% \newcommand{\Ib}{\mathbf{I}}
% \newcommand{\Jb}{\mathbf{J}}
% \newcommand{\Kb}{\mathbf{K}}
% \newcommand{\Lb}{\mathbf{L}}
% \newcommand{\Mb}{\mathbf{M}}
% \newcommand{\Nb}{\mathbf{N}}
% \newcommand{\Ob}{\mathbf{O}}
% \newcommand{\Pb}{\mathbf{P}}
% \newcommand{\Qb}{\mathbf{Q}}
% \newcommand{\Rb}{\mathbf{R}}
% \newcommand{\Sb}{\mathbf{S}}
% \newcommand{\Tb}{\mathbf{T}}
% \newcommand{\Ub}{\mathbf{U}}
% \newcommand{\Vb}{\mathbf{V}}
% \newcommand{\Wb}{\mathbf{W}}
% \newcommand{\Xb}{\mathbf{X}}
% \newcommand{\Yb}{\mathbf{Y}}
% \newcommand{\Zb}{\mathbf{Z}}

\newcommand{\abf}{\mathbf{a}}
\newcommand{\bbf}{\mathbf{b}}
\newcommand{\cbf}{\mathbf{c}}
\newcommand{\dbf}{\mathbf{d}}
\newcommand{\ebf}{\mathbf{e}}
\newcommand{\fbf}{\mathbf{f}}
\newcommand{\gbf}{\mathbf{g}}
\newcommand{\hbf}{\mathbf{h}}
\newcommand{\ibf}{\mathbf{i}}
\newcommand{\jbf}{\mathbf{j}}
\newcommand{\kbf}{\mathbf{k}}
\newcommand{\lbf}{\mathbf{l}}
\newcommand{\mbf}{\mathbf{m}}
\newcommand{\nbf}{\mathbf{n}}
\newcommand{\obf}{\mathbf{o}}
\newcommand{\pbf}{\mathbf{p}}
\newcommand{\qbf}{\mathbf{q}}
\newcommand{\rbf}{\mathbf{r}}
\newcommand{\sbf}{\mathbf{s}}
\newcommand{\tbf}{\mathbf{t}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\wbf}{\mathbf{w}}
\newcommand{\xbf}{\mathbf{x}}
\newcommand{\ybf}{\mathbf{y}}
\newcommand{\zbf}{\mathbf{z}}

% \renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Abf}
\newcommand{\Bmat}{\Bbf}
\newcommand{\Cmat}{\Cbf}
\newcommand{\Dmat}{\Dbf}
\newcommand{\Emat}{\Ebf}
\newcommand{\Fmat}{\Fbf}
\newcommand{\Gmat}{\Gbf}
\newcommand{\Hmat}{\Hbf}
\newcommand{\Imat}{\Ibf}
\newcommand{\Jmat}{\Jbf}
\newcommand{\Kmat}{\Kbf}
\newcommand{\Lmat}{\Lbf}
\newcommand{\Mmat}{\Mbf}
\newcommand{\Nmat}{\Nbf}
\newcommand{\Omat}{\Obf}
\newcommand{\Pmat}{\Pbf}
\newcommand{\Qmat}{\Qbf}
\newcommand{\Rmat}{\Rbf}
\newcommand{\Smat}{\Sbf}
\newcommand{\Tmat}{\Tbf}
\newcommand{\Umat}{\Ubf}
\newcommand{\Vmat}{\Vbf}
\newcommand{\Wmat}{\Wbf}
\newcommand{\Xmat}{\Xbf}
\newcommand{\Ymat}{\Ybf}
\newcommand{\Zmat}{\Zbf}

% mathrm
\newcommand{\Arm}{\mathrm{A}}
\newcommand{\Brm}{\mathrm{B}}
\newcommand{\Crm}{\mathrm{C}}
\newcommand{\Drm}{\mathrm{D}}
\newcommand{\Erm}{\mathrm{E}}
\newcommand{\Frm}{\mathrm{F}}
\newcommand{\Grm}{\mathrm{G}}
\newcommand{\Hrm}{\mathrm{H}}
\newcommand{\Irm}{\mathrm{I}}
\newcommand{\Jrm}{\mathrm{J}}
\newcommand{\Krm}{\mathrm{K}}
\newcommand{\Lrm}{\mathrm{L}}
\newcommand{\Mrm}{\mathrm{M}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\Orm}{\mathrm{O}}
\newcommand{\Prm}{\mathrm{P}}
\newcommand{\Qrm}{\mathrm{Q}}
\newcommand{\Rrm}{\mathrm{R}}
\newcommand{\Srm}{\mathrm{S}}
\newcommand{\Trm}{\mathrm{T}}
\newcommand{\Urm}{\mathrm{U}}
\newcommand{\Vrm}{\mathrm{V}}
\newcommand{\Wrm}{\mathrm{W}}
\newcommand{\Xrm}{\mathrm{X}}
\newcommand{\Yrm}{\mathrm{Y}}
\newcommand{\Zrm}{\mathrm{Z}}

\newcommand{\arm}{\mathrm{a}}
\newcommand{\brm}{\mathrm{b}}
\newcommand{\crm}{\mathrm{c}}
\newcommand{\drm}{\mathrm{d}}
\newcommand{\erm}{\mathrm{e}}
\newcommand{\frm}{\mathrm{f}}
\newcommand{\grm}{\mathrm{g}}
\newcommand{\hrm}{\mathrm{h}}
\newcommand{\irm}{\mathrm{i}}
\newcommand{\jrm}{\mathrm{j}}
\newcommand{\krm}{\mathrm{k}}
\newcommand{\lrm}{\mathrm{l}}
\newcommand{\mrm}{\mathrm{m}}
\newcommand{\nrm}{\mathrm{n}}
\newcommand{\orm}{\mathrm{o}}
\newcommand{\prm}{\mathrm{p}}
\newcommand{\qrm}{\mathrm{q}}
\newcommand{\rrm}{\mathrm{r}}
\newcommand{\srm}{\mathrm{s}}
\newcommand{\trm}{\mathrm{t}}
\newcommand{\urm}{\mathrm{u}}
\newcommand{\vrm}{\mathrm{v}}
\newcommand{\wrm}{\mathrm{w}}
\newcommand{\xrm}{\mathrm{x}}
\newcommand{\yrm}{\mathrm{y}}
\newcommand{\zrm}{\mathrm{z}}

% mathcal
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

% mathsf 
\newcommand{\Asf}{\mathsf{A}}
\newcommand{\Bsf}{\mathsf{B}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\Dsf}{\mathsf{D}}
\newcommand{\Esf}{\mathsf{E}}
\newcommand{\Fsf}{\mathsf{F}}
\newcommand{\Gsf}{\mathsf{G}}
\newcommand{\Hsf}{\mathsf{H}}
\newcommand{\Isf}{\mathsf{I}}
\newcommand{\Jsf}{\mathsf{J}}
\newcommand{\Ksf}{\mathsf{K}}
\newcommand{\Lsf}{\mathsf{L}}
\newcommand{\Msf}{\mathsf{M}}
\newcommand{\Nsf}{\mathsf{N}}
\newcommand{\Osf}{\mathsf{O}}
\newcommand{\Psf}{\mathsf{P}}
\newcommand{\Qsf}{\mathsf{Q}}
\newcommand{\Rsf}{\mathsf{R}}
\newcommand{\Ssf}{\mathsf{S}}
\newcommand{\Tsf}{\mathsf{T}}
\newcommand{\Usf}{\mathsf{U}}
\newcommand{\Vsf}{\mathsf{V}}
\newcommand{\Wsf}{\mathsf{W}}
\newcommand{\Xsf}{\mathsf{X}}
\newcommand{\Ysf}{\mathsf{Y}}
\newcommand{\Zsf}{\mathsf{Z}}

\newcommand{\asf}{\mathsf{a}}
\newcommand{\bsf}{\mathsf{b}}
\newcommand{\csf}{\mathsf{c}}
\newcommand{\dsf}{\mathsf{d}}
\newcommand{\esf}{\mathsf{e}}
\newcommand{\fsf}{\mathsf{f}}
\newcommand{\gsf}{\mathsf{g}}
\newcommand{\hsf}{\mathsf{h}}
\newcommand{\isf}{\mathsf{i}}
\newcommand{\jsf}{\mathsf{j}}
\newcommand{\ksf}{\mathsf{k}}
\newcommand{\lsf}{\mathsf{l}}
\newcommand{\msf}{\mathsf{m}}
\newcommand{\nsf}{\mathsf{n}}
\newcommand{\osf}{\mathsf{o}}
\newcommand{\psf}{\mathsf{p}}
\newcommand{\qsf}{\mathsf{q}}
\newcommand{\rsf}{\mathsf{r}}
\newcommand{\ssf}{\mathsf{s}}
\newcommand{\tsf}{\mathsf{t}}
\newcommand{\usf}{\mathsf{u}}
\newcommand{\vsf}{\mathsf{v}}
\newcommand{\wsf}{\mathsf{w}}
\newcommand{\xsf}{\mathsf{x}}
\newcommand{\ysf}{\mathsf{y}}
\newcommand{\zsf}{\mathsf{z}}

% mathtt
\newcommand{\Att}{\mathtt{A}}
\newcommand{\Btt}{\mathtt{B}}
\newcommand{\Ctt}{\mathtt{C}}
\newcommand{\Dtt}{\mathtt{D}}
\newcommand{\Ett}{\mathtt{E}}
\newcommand{\Ftt}{\mathtt{F}}
\newcommand{\Gtt}{\mathtt{G}}
\newcommand{\Htt}{\mathtt{H}}
\newcommand{\Itt}{\mathtt{I}}
\newcommand{\Jtt}{\mathtt{J}}
\newcommand{\Ktt}{\mathtt{K}}
\newcommand{\Ltt}{\mathtt{L}}
\newcommand{\Mtt}{\mathtt{M}}
\newcommand{\Ntt}{\mathtt{N}}
\newcommand{\Ott}{\mathtt{O}}
\newcommand{\Ptt}{\mathtt{P}}
\newcommand{\Qtt}{\mathtt{Q}}
\newcommand{\Rtt}{\mathtt{R}}
\newcommand{\Stt}{\mathtt{S}}
\newcommand{\Ttt}{\mathtt{T}}
\newcommand{\Utt}{\mathtt{U}}
\newcommand{\Vtt}{\mathtt{V}}
\newcommand{\Wtt}{\mathtt{W}}
\newcommand{\Xtt}{\mathtt{X}}
\newcommand{\Ytt}{\mathtt{Y}}
\newcommand{\Ztt}{\mathtt{Z}}

\newcommand{\att}{\mathtt{a}}
\newcommand{\btt}{\mathtt{b}}
\newcommand{\ctt}{\mathtt{c}}
\newcommand{\dtt}{\mathtt{d}}
\newcommand{\ett}{\mathtt{e}}
\newcommand{\ftt}{\mathtt{f}}
\newcommand{\gtt}{\mathtt{g}}
\newcommand{\htt}{\mathtt{h}}
\newcommand{\itt}{\mathtt{i}}
\newcommand{\jtt}{\mathtt{j}}
\newcommand{\ktt}{\mathtt{k}}
\newcommand{\ltt}{\mathtt{l}}
\newcommand{\mtt}{\mathtt{m}}
\newcommand{\ntt}{\mathtt{n}}
\newcommand{\ott}{\mathtt{o}}
\newcommand{\ptt}{\mathtt{p}}
\newcommand{\qtt}{\mathtt{q}}
\newcommand{\rtt}{\mathtt{r}}
\newcommand{\stt}{\mathtt{s}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\utt}{\mathtt{u}}
\newcommand{\vtt}{\mathtt{v}}
\newcommand{\wtt}{\mathtt{w}}
\newcommand{\xtt}{\mathtt{x}}
\newcommand{\ytt}{\mathtt{y}}
\newcommand{\ztt}{\mathtt{z}}

% mathit
\newcommand{\Ait}{\mathit{A}}
\newcommand{\Bit}{\mathit{B}}
\newcommand{\Cit}{\mathit{C}}
\newcommand{\Dit}{\mathit{D}}
\newcommand{\Eit}{\mathit{E}}
\newcommand{\Fit}{\mathit{F}}
\newcommand{\Git}{\mathit{G}}
\newcommand{\Hit}{\mathit{H}}
\newcommand{\Iit}{\mathit{I}}
\newcommand{\Jit}{\mathit{J}}
\newcommand{\Kit}{\mathit{K}}
\newcommand{\Lit}{\mathit{L}}
\newcommand{\Mit}{\mathit{M}}
\newcommand{\Nit}{\mathit{N}}
\newcommand{\Oit}{\mathit{O}}
\newcommand{\Pit}{\mathit{P}}
\newcommand{\Qit}{\mathit{Q}}
\newcommand{\Rit}{\mathit{R}}
\newcommand{\Sit}{\mathit{S}}
\newcommand{\Tit}{\mathit{T}}
\newcommand{\Uit}{\mathit{U}}
\newcommand{\Vit}{\mathit{V}}
\newcommand{\Wit}{\mathit{W}}
\newcommand{\Xit}{\mathit{X}}
\newcommand{\Yit}{\mathit{Y}}
\newcommand{\Zit}{\mathit{Z}}

\newcommand{\ait}{\mathit{a}}
\newcommand{\bit}{\mathit{b}}
\newcommand{\cit}{\mathit{c}}
\newcommand{\dit}{\mathit{d}}
\newcommand{\eit}{\mathit{e}}
\newcommand{\fit}{\mathit{f}}
\newcommand{\git}{\mathit{g}}
\newcommand{\hit}{\mathit{h}}
\newcommand{\iit}{\mathit{i}}
\newcommand{\jit}{\mathit{j}}
\newcommand{\kit}{\mathit{k}}
\newcommand{\lit}{\mathit{l}}
\newcommand{\itm}{\mathit{m}} % \mit is already defined
\renewcommand{\mit}{\mathit{m}}
\newcommand{\nit}{\mathit{n}}
\newcommand{\oit}{\mathit{o}}
\newcommand{\pit}{\mathit{p}}
\newcommand{\qit}{\mathit{q}}
\newcommand{\rit}{\mathit{r}}
\newcommand{\sit}{\mathit{s}}
\newcommand{\tit}{\mathit{t}}
\newcommand{\uit}{\mathit{u}}
\newcommand{\vit}{\mathit{v}}
\newcommand{\wit}{\mathit{w}}
\newcommand{\xit}{\mathit{x}}
\newcommand{\yit}{\mathit{y}}
\newcommand{\zit}{\mathit{z}}

% mathfrak
\newcommand{\afk}{\mathfrak{a}}
\newcommand{\bfk}{\mathfrak{b}}
\newcommand{\cfk}{\mathfrak{c}}
\newcommand{\dfk}{\mathfrak{d}}
\newcommand{\efk}{\mathfrak{e}}
\newcommand{\ffk}{\mathfrak{f}}
\newcommand{\gfk}{\mathfrak{g}}
\newcommand{\hfk}{\mathfrak{h}}
\newcommand{\ifk}{\mathfrak{i}}
\newcommand{\jfk}{\mathfrak{j}}
\newcommand{\kfk}{\mathfrak{k}}
\newcommand{\lfk}{\mathfrak{l}}
\newcommand{\mfk}{\mathfrak{m}}
\newcommand{\nfk}{\mathfrak{n}}
\newcommand{\ofk}{\mathfrak{o}}
\newcommand{\pfk}{\mathfrak{p}}
\newcommand{\qfk}{\mathfrak{q}}
\newcommand{\rfk}{\mathfrak{r}}
\newcommand{\sfk}{\mathfrak{s}}
\newcommand{\tfk}{\mathfrak{t}}
\newcommand{\ufk}{\mathfrak{u}}
\newcommand{\vfk}{\mathfrak{v}}
\newcommand{\wfk}{\mathfrak{w}}
\newcommand{\xfk}{\mathfrak{x}}
\newcommand{\yfk}{\mathfrak{y}}
\newcommand{\zfk}{\mathfrak{z}}

\newcommand{\Afk}{\mathfrak{A}}
\newcommand{\Bfk}{\mathfrak{B}}
\newcommand{\Cfk}{\mathfrak{C}}
\newcommand{\Dfk}{\mathfrak{D}}
\newcommand{\Efk}{\mathfrak{E}}
\newcommand{\Ffk}{\mathfrak{F}}
\newcommand{\Gfk}{\mathfrak{G}}
\newcommand{\Hfk}{\mathfrak{H}}
\newcommand{\Ifk}{\mathfrak{I}}
\newcommand{\Jfk}{\mathfrak{J}}
\newcommand{\Kfk}{\mathfrak{K}}
\newcommand{\Lfk}{\mathfrak{L}}
\newcommand{\Mfk}{\mathfrak{M}}
\newcommand{\Nfk}{\mathfrak{N}}
\newcommand{\Ofk}{\mathfrak{O}}
\newcommand{\Pfk}{\mathfrak{P}}
\newcommand{\Qfk}{\mathfrak{Q}}
\newcommand{\Rfk}{\mathfrak{R}}
\newcommand{\Sfk}{\mathfrak{S}}
\newcommand{\Tfk}{\mathfrak{T}}
\newcommand{\Ufk}{\mathfrak{U}}
\newcommand{\Vfk}{\mathfrak{V}}
\newcommand{\Wfk}{\mathfrak{W}}
\newcommand{\Xfk}{\mathfrak{X}}
\newcommand{\Yfk}{\mathfrak{Y}}
\newcommand{\Zfk}{\mathfrak{Z}}

% mathbb
\newcommand{\Abb}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}} % \Bbb is already defined in amssymb
\renewcommand{\Bbb}{\mathbb{B}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Dbb}{\mathbb{D}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jbb}{\mathbb{J}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Lbb}{\mathbb{L}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Qbb}{\mathbb{Q}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Tbb}{\mathbb{T}}
\newcommand{\Ubb}{\mathbb{U}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Wbb}{\mathbb{W}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}

% mathds
\newcommand{\Ads}{\mathds{A}}
\newcommand{\Bds}{\mathds{B}}
\newcommand{\Cds}{\mathds{C}}
\newcommand{\Dds}{\mathds{D}}
\newcommand{\Eds}{\mathds{E}}
\newcommand{\Fds}{\mathds{F}}
\newcommand{\Gds}{\mathds{G}}
\newcommand{\Hds}{\mathds{H}}
\newcommand{\Ids}{\mathds{I}}
\newcommand{\Jds}{\mathds{J}}
\newcommand{\Kds}{\mathds{K}}
\newcommand{\Lds}{\mathds{L}}
\newcommand{\Mds}{\mathds{M}}
\newcommand{\Nds}{\mathds{N}}
\newcommand{\Ods}{\mathds{O}}
\newcommand{\Pds}{\mathds{P}}
\newcommand{\Qds}{\mathds{Q}}
\newcommand{\Rds}{\mathds{R}}
\newcommand{\Sds}{\mathds{S}}
\newcommand{\Tds}{\mathds{T}}
\newcommand{\Uds}{\mathds{U}}
\newcommand{\Vds}{\mathds{V}}
\newcommand{\Wds}{\mathds{W}}
\newcommand{\Xds}{\mathds{X}}
\newcommand{\Yds}{\mathds{Y}}
\newcommand{\Zds}{\mathds{Z}}

% mathscr
\newcommand{\As}{\mathscr{A}}
\newcommand{\Bs}{\mathscr{B}}
\newcommand{\Cs}{\mathscr{C}}
\newcommand{\Ds}{\mathscr{D}}
\newcommand{\Es}{\mathscr{E}}
\newcommand{\Fs}{\mathscr{F}}
\newcommand{\Gs}{\mathscr{G}}
\newcommand{\Hs}{\mathscr{H}}
\newcommand{\Is}{\mathscr{I}}
\newcommand{\Js}{\mathscr{J}}
\newcommand{\Ks}{\mathscr{K}}
\newcommand{\Ls}{\mathscr{L}}
\newcommand{\Ms}{\mathscr{M}}
\newcommand{\Ns}{\mathscr{N}}
\newcommand{\Os}{\mathscr{O}}
\newcommand{\Ps}{\mathscr{P}}
\newcommand{\Qs}{\mathscr{Q}}
\newcommand{\Rs}{\mathscr{R}}
\newcommand{\Ss}{\mathscr{S}}
\newcommand{\Ts}{\mathscr{T}}
\newcommand{\Us}{\mathscr{U}}
\newcommand{\Vs}{\mathscr{V}}
\newcommand{\Ws}{\mathscr{W}}
\newcommand{\Xs}{\mathscr{X}}
\newcommand{\Ys}{\mathscr{Y}}
\newcommand{\Zs}{\mathscr{Z}}

%%%%%%%%%%%%% Math Accents %%%%%%%%%%%%%%%%%%%
% tilde
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

% wildetilde
\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

% hat
\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

% bar
\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\renewcommand{\hbar}{\bar{h}} % \hbar is already defined
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

%%%%%%%%%%%%% Combinations of fonts and accents %%%%%%%%%%%%%%%%%%%
% mathbf + tilde
\newcommand{\abtil}{\tilde{\abf}}
\newcommand{\bbtil}{\tilde{\bbf}}
\newcommand{\cbtil}{\tilde{\cbf}}
\newcommand{\dbtil}{\tilde{\dbf}}
\newcommand{\ebtil}{\tilde{\ebf}}
\newcommand{\fbtil}{\tilde{\fbf}}
\newcommand{\gbtil}{\tilde{\gbf}}
\newcommand{\hbtil}{\tilde{\hbf}}
\newcommand{\ibtil}{\tilde{\ibf}}
\newcommand{\jbtil}{\tilde{\jbf}}
\newcommand{\kbtil}{\tilde{\kbf}}
\newcommand{\lbtil}{\tilde{\lbf}}
\newcommand{\mbtil}{\tilde{\mbf}}
\newcommand{\nbtil}{\tilde{\nbf}}
\newcommand{\obtil}{\tilde{\obf}}
\newcommand{\pbtil}{\tilde{\pbf}}
\newcommand{\qbtil}{\tilde{\qbf}}
\newcommand{\rbtil}{\tilde{\rbf}}
\newcommand{\sbtil}{\tilde{\sbf}}
\newcommand{\tbtil}{\tilde{\tbf}}
\newcommand{\ubtil}{\tilde{\ubf}}
\newcommand{\vbtil}{\tilde{\vbf}}
\newcommand{\wbtil}{\tilde{\wbf}}
\newcommand{\xbtil}{\tilde{\xbf}}
\newcommand{\ybtil}{\tilde{\ybf}}
\newcommand{\zbtil}{\tilde{\zbf}}

\newcommand{\Abtil}{\tilde{\Abf}}
\newcommand{\Bbtil}{\tilde{\Bbf}}
\newcommand{\Cbtil}{\tilde{\Cbf}}
\newcommand{\Dbtil}{\tilde{\Dbf}}
\newcommand{\Ebtil}{\tilde{\Ebf}}
\newcommand{\Fbtil}{\tilde{\Fbf}}
\newcommand{\Gbtil}{\tilde{\Gbf}}
\newcommand{\Hbtil}{\tilde{\Hbf}}
\newcommand{\Ibtil}{\tilde{\Ibf}}
\newcommand{\Jbtil}{\tilde{\Jbf}}
\newcommand{\Kbtil}{\tilde{\Kbf}}
\newcommand{\Lbtil}{\tilde{\Lbf}}
\newcommand{\Mbtil}{\tilde{\Mbf}}
\newcommand{\Nbtil}{\tilde{\Nbf}}
\newcommand{\Obtil}{\tilde{\Obf}}
\newcommand{\Pbtil}{\tilde{\Pbf}}
\newcommand{\Qbtil}{\tilde{\Qbf}}
\newcommand{\Rbtil}{\tilde{\Rbf}}
\newcommand{\Sbtil}{\tilde{\Sbf}}
\newcommand{\Tbtil}{\tilde{\Tbf}}
\newcommand{\Ubtil}{\tilde{\Ubf}}
\newcommand{\Vbtil}{\tilde{\Vbf}}
\newcommand{\Wbtil}{\tilde{\Wbf}}
\newcommand{\Xbtil}{\tilde{\Xbf}}
\newcommand{\Ybtil}{\tilde{\Ybf}}
\newcommand{\Zbtil}{\tilde{\Zbf}}

% mathbf + hat
\newcommand{\abhat}{\hat{\abf}}
\newcommand{\bbhat}{\hat{\bbf}}
\newcommand{\cbhat}{\hat{\cbf}}
\newcommand{\dbhat}{\hat{\dbf}}
\newcommand{\ebhat}{\hat{\ebf}}
\newcommand{\fbhat}{\hat{\fbf}}
\newcommand{\gbhat}{\hat{\gbf}}
\newcommand{\hbhat}{\hat{\hbf}}
\newcommand{\ibhat}{\hat{\ibf}}
\newcommand{\jbhat}{\hat{\jbf}}
\newcommand{\kbhat}{\hat{\kbf}}
\newcommand{\lbhat}{\hat{\lbf}}
\newcommand{\mbhat}{\hat{\mbf}}
\newcommand{\nbhat}{\hat{\nbf}}
\newcommand{\obhat}{\hat{\obf}}
\newcommand{\pbhat}{\hat{\pbf}}
\newcommand{\qbhat}{\hat{\qbf}}
\newcommand{\rbhat}{\hat{\rbf}}
\newcommand{\sbhat}{\hat{\sbf}}
\newcommand{\tbhat}{\hat{\tbf}}
\newcommand{\ubhat}{\hat{\ubf}}
\newcommand{\vbhat}{\hat{\vbf}}
\newcommand{\wbhat}{\hat{\wbf}}
\newcommand{\xbhat}{\hat{\xbf}}
\newcommand{\ybhat}{\hat{\ybf}}
\newcommand{\zbhat}{\hat{\zbf}}

\newcommand{\Abhat}{\hat{\Abf}}
\newcommand{\Bbhat}{\hat{\Bbf}}
\newcommand{\Cbhat}{\hat{\Cbf}}
\newcommand{\Dbhat}{\hat{\Dbf}}
\newcommand{\Ebhat}{\hat{\Ebf}}
\newcommand{\Fbhat}{\hat{\Fbf}}
\newcommand{\Gbhat}{\hat{\Gbf}}
\newcommand{\Hbhat}{\hat{\Hbf}}
\newcommand{\Ibhat}{\hat{\Ibf}}
\newcommand{\Jbhat}{\hat{\Jbf}}
\newcommand{\Kbhat}{\hat{\Kbf}}
\newcommand{\Lbhat}{\hat{\Lbf}}
\newcommand{\Mbhat}{\hat{\Mbf}}
\newcommand{\Nbhat}{\hat{\Nbf}}
\newcommand{\Obhat}{\hat{\Obf}}
\newcommand{\Pbhat}{\hat{\Pbf}}
\newcommand{\Qbhat}{\hat{\Qbf}}
\newcommand{\Rbhat}{\hat{\Rbf}}
\newcommand{\Sbhat}{\hat{\Sbf}}
\newcommand{\Tbhat}{\hat{\Tbf}}
\newcommand{\Ubhat}{\hat{\Ubf}}
\newcommand{\Vbhat}{\hat{\Vbf}}
\newcommand{\Wbhat}{\hat{\Wbf}}
\newcommand{\Xbhat}{\hat{\Xbf}}
\newcommand{\Ybhat}{\hat{\Ybf}}
\newcommand{\Zbhat}{\hat{\Zbf}}

% mathbf + bar
\newcommand{\abbar}{\bar{\abf}}
\newcommand{\bbbar}{\bar{\bbf}}
\newcommand{\cbbar}{\bar{\cbf}}
\newcommand{\dbbar}{\bar{\dbf}}
\newcommand{\ebbar}{\bar{\ebf}}
\newcommand{\fbbar}{\bar{\fbf}}
\newcommand{\gbbar}{\bar{\gbf}}
\newcommand{\hbbar}{\bar{\hbf}}
\newcommand{\ibbar}{\bar{\ibf}}
\newcommand{\jbbar}{\bar{\jbf}}
\newcommand{\kbbar}{\bar{\kbf}}
\newcommand{\lbbar}{\bar{\lbf}}
\newcommand{\mbbar}{\bar{\mbf}}
\newcommand{\nbbar}{\bar{\nbf}}
\newcommand{\obbar}{\bar{\obf}}
\newcommand{\pbbar}{\bar{\pbf}}
\newcommand{\qbbar}{\bar{\qbf}}
\newcommand{\rbbar}{\bar{\rbf}}
\newcommand{\sbbar}{\bar{\sbf}}
\newcommand{\tbbar}{\bar{\tbf}}
\newcommand{\ubbar}{\bar{\ubf}}
\newcommand{\vbbar}{\bar{\vbf}}
\newcommand{\wbbar}{\bar{\wbf}}
\newcommand{\xbbar}{\bar{\xbf}}
\newcommand{\ybbar}{\bar{\ybf}}
\newcommand{\zbbar}{\bar{\zbf}}

\newcommand{\Abbar}{\bar{\Abf}}
\newcommand{\Bbbar}{\bar{\Bbf}}
\newcommand{\Cbbar}{\bar{\Cbf}}
\newcommand{\Dbbar}{\bar{\Dbf}}
\newcommand{\Ebbar}{\bar{\Ebf}}
\newcommand{\Fbbar}{\bar{\Fbf}}
\newcommand{\Gbbar}{\bar{\Gbf}}
\newcommand{\Hbbar}{\bar{\Hbf}}
\newcommand{\Ibbar}{\bar{\Ibf}}
\newcommand{\Jbbar}{\bar{\Jbf}}
\newcommand{\Kbbar}{\bar{\Kbf}}
\newcommand{\Lbbar}{\bar{\Lbf}}
\newcommand{\Mbbar}{\bar{\Mbf}}
\newcommand{\Nbbar}{\bar{\Nbf}}
\newcommand{\Obbar}{\bar{\Obf}}
\newcommand{\Pbbar}{\bar{\Pbf}}
\newcommand{\Qbbar}{\bar{\Qbf}}
\newcommand{\Rbbar}{\bar{\Rbf}}
\newcommand{\Sbbar}{\bar{\Sbf}}
\newcommand{\Tbbar}{\bar{\Tbf}}
\newcommand{\Ubbar}{\bar{\Ubf}}
\newcommand{\Vbbar}{\bar{\Vbf}}
\newcommand{\Wbbar}{\bar{\Wbf}}
\newcommand{\Xbbar}{\bar{\Xbf}}
\newcommand{\Ybbar}{\bar{\Ybf}}
\newcommand{\Zbbar}{\bar{\Zbf}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

% \renewcommand{\qedsymbol}{$\blacksquare$}

\ifx\BlackBox\undefined
  \newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
  \def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
  \newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.0mm]}
  % \newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
  \newtheorem{theorem}{Theorem}
  % \newtheorem{theorem}{Theorem}[section]
\fi

\ifx\example\undefined
  \newtheorem{example}{Example}
\fi

\ifx\property\undefined
  \newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
  \newtheorem{lemma}{Lemma}
\fi

\ifx\proposition\undefined
  \newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
  \newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
  \newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
  \newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
  \newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
  \newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
  \newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
  \newtheorem{assumption}{Assumption}
  % \newtheorem{assumption}{Postulate}
\fi

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%

\newcommand{\CC}{\mathds{C}}                      % Complex numbers
\newcommand{\EE}{\mathsf{E}}                      % Expectation
\newcommand{\FF}{\mathds{F}}                      % Arbitrary field
\newcommand{\HH}{\mathsf{H}}                      % Entropy
\newcommand{\id}{\mathsf{Id}}                     % Identity
\newcommand{\KK}{\mathds{K}}                      % Arbitrary field
\newcommand{\MM}{\mathsf{M}}                      % Median
\newcommand{\NN}{\mathds{N}}                      % Natural numbers
\newcommand{\PP}{\mathsf{P}}                      % Probability
\newcommand{\QQ}{\mathds{Q}}                      % Rationals
\newcommand{\RR}{\mathds{R}}                      % Real numbers
\newcommand{\RRbar}{\overline{\RR}}               % Real numbers
\newcommand{\RRi}{\RR_{\infty}}                   % Real numbers
\newcommand{\VV}{\mathsf{Var}}                    % Variance
\newcommand{\ZZ}{\mathds{Z}}                      % Integers
\newcommand{\pp}{\mathsf{p}}                      % density
\newcommand{\MI}{\mathsf{MI}}                     % Mutual Information

%%%%%%%% Mathematical Operations %%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}   % minimize
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}   % maximize
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}   % argmin
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}   % argmax
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}   % arginf
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}   % argsup
\newcommand{\sgn}{\mathop{\mathrm{sign}}}         % sign
\newcommand{\tr}{\mathop{\mathrm{tr}}}            % trace
\newcommand{\diag}{\mathop{\mathrm{diag}}}        % diagonal
\newcommand{\rank}{\mathop{\mathrm{rank}}}        % rank
\newcommand{\vect}{\mathop{\mathrm{vec}}}         % vectorize
\newcommand{\traj}{\mathop{\mathrm{Traj}}}        % trajectory
\newcommand{\cov}{\mathrm{Cov}}                   % covariance
\newcommand{\conv}{\mathrm{conv\,}}               % convex cone
\newcommand{\cone}{\mathrm{cone\,}}               % conic hull
\newcommand{\const}{\mathrm{constant}}            % constant
\newcommand{\dom}{\mathop{\mathrm{dom}}}          % domain
\newcommand{\ri}{\mathop{\mathrm{ri}}}            % relative interior
\newcommand{\sri}{\mathop{\mathrm{sri}}}          % strict relative interior
\newcommand{\cl}{\mathop{\mathrm{cl}}}            % closure
\newcommand{\intr}{\mathop{\mathrm{int}}}         % interior
\newcommand{\bd}{\mathop{\mathrm{bd}}}            % boundary
\newcommand{\emp}{\mathop{\mathrm{emp}}}          % empirical
\newcommand{\core}{\mathop{\mathrm{core}}}        % core
\newcommand{\epi}{\mathop{\mathrm{epi}}}          % epigraph
\newcommand{\co}{\mathop{\mathrm{co}}}            % convex hull
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}          % nonzeros  
\newcommand{\med}{\mathop{\mathrm{med}}}          % median
\newcommand{\eproof}{$\null\hfill\blacksquare$}   % end of proof
% \newcommand{\ln}{\mathop{\mathrm{ln}}}            % logrithm base on e, not \log base on 10


%%%%%%%% Short Forms %%%%%%%%
\newcommand{\ea}{{et al.}\xspace}   % et al.
\newcommand{\eg}{{e.g.}\xspace}     % e.g.
\newcommand{\ie}{{i.e.}\xspace}     % i.e.
\newcommand{\iid}{{i.i.d.}\xspace}  % i.i.d.
\newcommand{\cf}{{cf.}\xspace}      % cf.
\newcommand{\wrt}{{w.r.t.}\xspace}  % w.r.t.
\newcommand{\aka}{{a.k.a.}\xspace}  % a.k.a.
\newcommand{\etc}{{etc.}\xspace}    % etc.

%%%%%%%% Brackets %%%%%%%%
\newcommand{\rbr}[1]{\left(#1\right)}                     % round brackets
\newcommand{\sbr}[1]{\left[#1\right]}                     % square brackets
\newcommand{\cbr}[1]{\left\{#1\right\}}                   % curly brackets
\newcommand{\nbr}[1]{\left\|#1\right\|}                   % norm brackets
\newcommand{\abr}[1]{\left|#1\right|}                     % absolute brackets
\newcommand{\abs}[1]{\left|#1\right|}                     % absolute brackets
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}     % floor brackets
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}        % ceiling brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}  % inner product
\newcommand{\dual}[2]{\left\langle #1;#2 \right\rangle}   % dual product
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}                    % triple norm
\newcommand{\sembrack}[1]{[\![#1]\!]}                     % semantic brackets
\newcommand{\norm}[1]{\left\|#1\right\|}                  % norm
\newcommand{\dualnorm}[1]{\left\|#1\right\|_{\circ}}      % dual norm

%%%%%%%%  Mathematical Constants  %%%%%%%%
\newcommand{\one}{\mathbf{1}}                 % bold one
\newcommand{\zero}{\mathbf{0}}                % bold zero
\newcommand{\half}{\frac{1}{2}}               % fraction 1/2
\newcommand{\sqrttwo}{\sqrt{2}}               % sqrt(2)  
\newcommand{\shalf}{\textstyle\frac{1}{2}}    % small fraction 1/2
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}  % 1/sqrt(2)
\newcommand*\rmd{\mathop{}\!\mathrm{d}}       % roman d
\newcommand{\poly}[1][P]{\mathfrak{#1}}       % polynomial
\newcommand{\face}[1][F]{\mathfrak{#1}}       % face

%%%%%%%% Utility functions %%%%%%%%
\newcommand{\eq}[1]{(\ref{#1})}                                                 % ref equation
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}        % compact matrix
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}   % row matrix
\newcommand{\mydet}[1]{\det\left[ #1 \right]}                                   % determinant
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}                                  % span
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}                          % small fraction
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}                             % first order partial derivative
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}                      % second order partial derivative
\newcommand{\aleq}{\preccurlyeq}                                                % almost less than
\newcommand{\ageq}{\succcurlyeq}

% todo: double check the following commands
\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}
\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\vardef}{\stackrel{\triangle}{=}}

%%%%%%%% Greek Symbols %%%%%%%%

% ! rename var 
% \newcommand{\ve}{\varepsilon}
% \newcommand{\vt}{\vartheta}
% \newcommand{\vs}{\varsigma}
% \newcommand{\vr}{\varrho}
% \newcommand{\vphi}{\varphi}
% \newcommand{\vpsi}{\varpsi}

% bold lowercase greek 
\newcommand{\alphavec}{\vec{\alpha}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\epsilonvec}{\vec{\epsilon}}
\newcommand{\varepsilonvec}{\vec{\varepsilon}}
\newcommand{\zetavec}{\vec{\zeta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\varthetavec}{\vec{\vartheta}}
\newcommand{\iotavec}{\vec{\iota}}
\newcommand{\kappavec}{\vec{\kappa}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\nuvec}{\vec{\nu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\pivec}{\vec{\pi}}
\newcommand{\varpivec}{\vec{\varpi}}
\newcommand{\rhovec}{\vec{\rho}}
\newcommand{\varrhovec}{\vec{\varrho}}
\newcommand{\sigmavec}{\vec{\sigma}}
\newcommand{\varsigmavec}{\vec{\varsigma}}
\newcommand{\tauvec}{\vec{\tau}}
\newcommand{\upsilonvec}{\vec{\upsilon}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\varphivec}{\vec{\varphi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\omegavec}{\vec{\omega}}

% bold uppercase greek
\newcommand{\Alphavec}{\vec{\Alpha}}
\newcommand{\Betavec}{\vec{\Beta}}
\newcommand{\Gammavec}{\vec{\Gamma}}
\newcommand{\Deltavec}{\vec{\Delta}}
\newcommand{\Epsilonvec}{\vec{\Epsilon}}
\newcommand{\Zetavec}{\vec{\Zeta}}
\newcommand{\Etavec}{\vec{\Eta}}
\newcommand{\Thetavec}{\vec{\Theta}}
\newcommand{\Iotavec}{\vec{\Iota}}
\newcommand{\Kappavec}{\vec{\Kappa}}
\newcommand{\Lambdavec}{\vec{\Lambda}}
\newcommand{\Muvec}{\vec{\Mu}}
\newcommand{\Nuvec}{\vec{\Nu}}
\newcommand{\Xivec}{\vec{\Xi}}
\newcommand{\Pivec}{\vec{\Pi}}
\newcommand{\Rhovec}{\vec{\Rho}}
\newcommand{\Sigamavec}{\vec{\Sigma}}
\newcommand{\Tauvec}{\vec{\Tau}}
\newcommand{\Upsilonvec}{\vec{\Upsilon}}
\newcommand{\Phivec}{\vec{\Phi}}
\newcommand{\Chivec}{\vec{\Chi}}
\newcommand{\Psivec}{\vec{\Psi}}
\newcommand{\Omegavec}{\vec{\Omega}}




% \newcommand{\gstar}{g^{\star}}
% \newcommand{\fstar}{f^{\star}}
% \newcommand{\hstar}{h^{\star}}
% \newcommand{\Astar}{A^{\star}}
% \newcommand{\Kstar}{K^{\star}}



% \newcommand{\Aone}{\textbf{A1}}
% \newcommand{\Atwo}{\textbf{A2}}
% \newcommand{\supp}{\mathrm{supp}}
% \newcommand{\blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
% \newcommand{\red}[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
% \newcommand{\green}[1]{\textcolor[rgb]{0.00,1.00,0.00}{#1}}
% \newcommand{\black}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
% \newcommand{\smallonevec}{{\scriptsize\mathbf 1}}
% \newcommand{\smallwvec}{{\scriptsize\mathbf w}}
% \newcommand{\smallqvec}{{\scriptsize\mathbf q}}
% \newcommand{\smallyvec}{{\scriptsize\mathbf y}}
% \newcommand{\smallepsvec}{{\mbox{\boldmath\scriptsize $\epsilon$}}}
% \newcommand{\smallzetavec}{{\mbox{\boldmath\scriptsize $\zeta$}}}
% \newcommand{\smallmuvec}{{\mbox{\boldmath\scriptsize $\mu$}}}
% \newcommand{\smallnuvec}{{\mbox{\boldmath\scriptsize $\nu$}}}
% \newcommand{\smallxivec}{{\mbox{\boldmath\scriptsize $\xi$}}}
% \newcommand{\smalllambdavec}{{\mbox{\boldmath\scriptsize $\lambda$}}}
% \newcommand{\smallthetavec}{{\mbox{\boldmath\scriptsize $\theta$}}}
% \newcommand{\smallalphavec}{{\mbox{\boldmath\scriptsize $\alpha$}}}
% \newcommand{\smallbetavec}{{\mbox{\boldmath\scriptsize $\beta$}}}
% \newcommand{\smalletavec}{{\mbox{\boldmath\scriptsize $\eta$}}}
% \newcommand{\smallomegavec}{{\mbox{\boldmath\scriptsize $\omega$}}}
% \newcommand{\smallLambdavec}{{\mbox{\boldmath\scriptsize $\Lambda$}}}

% \newcommand{\ellvec}{{\mbox{\boldmath $\ell$}}}
% \newcommand{\sign}{{\textrm{sign}}}
% \newcommand{\hinge}{{\textit{hinge}}}
% \newcommand{\loss}{{\textit{loss}}}
% \newcommand{\etahinge}[1]{{{#1}\mbox{-}\hinge}}
% \newcommand{\robust}{{\textit{robust}}}
% %\newcommand{\regrobust}{{f_{\scriptsize\textit{robust}}}}
% \newcommand{\regrobust}{{f_{\scriptsize\textit{rob}}}}
% %\newcommand{\regetahinge}{{f_{\scriptsize\textit{hinge}}}}
% \newcommand{\regetahinge}{{f_{\scriptsize\textit{hng}}}}
% \newcommand{\looerr}{{\textit{loo\_err}}}
% \newcommand{\makevector}[1]{{\mathbf #1}}
% \newcommand{\zerovec}{{\makevector{0}}}

% \newcommand{\cc}[1]{\mathrm{\overline{conv}}#1}
% \newcommand{\qcc}[1]{\mathrm{\overline{qconv}}#1}
% \newcommand{\Diag}{\mathrm{Diag}}
% \newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
% \newcommand{\Img}{\ensuremath{\mathrm{Im}}}
% %\renewcommand*{\theHsection}{\thesection}
% %\newcommand{\theHalgorithm}{\arabic{algorithm}}
% %\renewcommand{\qedsymbol}{$\blacksquare$}
% \newcommand{\Ball}[1]{\mathsf{B}_{#1}}
% \newcommand{\st}{\mathrm{s.t.}}
% \newcommand{\ran}{\mathrm{ran}}
% \newcommand{\qq}{\mathsf{q}}
% \newcommand{\ccp}{\Gamma_0}
% \newcommand{\tv}{\mathsf{TV}}
% \newcommand{\fl}{\mathsf{FL}}
% \newcommand{\gl}{\mathsf{GL}}
% \newcommand{\env}[2][\eta]{\mathsf{M}^{#1}_{#2}}
% \newcommand{\SC}[1][\eta]{\mathsf{SC}_{#1}}
% \renewcommand{\SS}[1][\eta]{\mathsf{SS}_{1/#1}}
% \newcommand{\prox}[2][\eta]{\mathsf{P}^{#1}_{#2}}
% \newcommand{\pa}[1][\eta]{\mathsf{A}^{#1}}
% \newcommand{\Ltwobar}{\overline{M^2}}
% \newcommand{\rse}{{RSE}}
% \newcommand{\nnzc}{{\mathrm{nnzc}}}
% \newcommand{\proj}{{\mathop{\mathrm{proj}}}}
% \newcommand{\Dsq}{{D_{\text{sq}}}}
% \newcommand{\Dent}{{D_{\text{ent}}}}
% \newcommand{\Fsq}{{F_{\text{sq}}}}
% \newcommand{\Fent}{{F_{\text{ent}}}}
% \newcommand{\sigmasq}{{\sigma_{\text{sq}}}}
% \newcommand{\sigmaent}{{\sigma_{\text{ent}}}}
% \newcommand{\Diamsq}{{\mathrm{D}}_{\text{sq}}}
% \newcommand{\Diament}{{\mathrm{D}}_{\text{ent}}}
% \newcommand{\Msq}{{\mathrm{M}}_{\text{sq}}}
% \newcommand{\Ment}{{\mathrm{M}}_{\text{ent}}}
% \newcommand{\sigmasqhat}{{\sigmahat_{\text{sq}}}}
% \newcommand{\sigmaenthat}{{\sigmahat_{\text{ent}}}}
% \newcommand{\Diamsqhat}{{\mathrm{\Dhat}}_{\text{sq}}}
% \newcommand{\Diamenthat}{{\mathrm{\Dhat}}_{\text{ent}}}
% \newcommand{\Msqhat}{{\mathrm{\Mhat}}_{\text{sq}}}
% \newcommand{\Menthat}{{\mathrm{\Mhat}}_{\text{ent}}}
% \newcommand{\Gsfhat}{{\hat{\Gsf}}}

% \newcommand{\sigmamin}{{\sigma_{\text{min}}}}
% \newcommand{\colspan}{{\text{col-span}}}
% \newcommand{\colker}{{\text{col-kernel}}}

%%%%%%%% User defined %%%%%%%%
% \newcommand{\note}[1]{{\color{red} #1}}

% \newcommand{\yvecbar}{\bar{\vec{y}}}
% \newcommand{\wvecbar}{\bar{\vec{w}}}
% \newcommand{\xvecbar}{\bar{\vec{x}}}
% \newcommand{\yvectil}{\tilde{\vec{y}}}
% \newcommand{\yvechat}{\hat{\vec{y}}}
% \newcommand{\gvechat}{\hat{\vec{g}}}
% \newcommand{\hvechat}{\hat{\vec{h}}}










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\val}{\vec{\alpha}}
% \newcommand{\vbeta}{\vec{\beta}}
% \newcommand{\vga}{\vec{\gamma}}
% \newcommand{\vde}{\vec{\delta}}
% \newcommand{\veps}{\vec{\epsilon}}
% \newcommand{\vveps}{\vec{\varepsilon}}
% \newcommand{\vze}{\vec{\zeta}}
% \newcommand{\veta}{\vec{\eta}}
% \newcommand{\vth}{\vec{\theta}}
% \newcommand{\vvth}{\vec{\vartheta}}
% \newcommand{\viota}{\vec{\iota}}
% \newcommand{\vkappa}{\vec{\kappa}}
% \newcommand{\vlambda}{\vec{\lambda}}
% \newcommand{\vmu}{\vec{\mu}}
% \newcommand{\vnu}{\vec{\nu}}
% \newcommand{\vxi}{\vec{\xi}}
% \newcommand{\vpi}{\vec{\pi}}
% \newcommand{\vvpi}{\vec{\varpi}}
% \newcommand{\vrho}{\vec{\rho}}
% \newcommand{\vvrho}{\vec{\varrho}}
% \newcommand{\vsig}{\vec{\sigma}}
% \newcommand{\vvsig}{\vec{\varsigma}}
% \newcommand{\vtau}{\vec{\tau}}
% \newcommand{\vups}{\vec{\upsilon}}
% \newcommand{\vphi}{\vec{\phi}}
% \newcommand{\vvphi}{\vec{\varphi}}
% \newcommand{\vchi}{\vec{\chi}}
% \newcommand{\vpsi}{\vec{\psi}}
% \newcommand{\vom}{\vec{\omega}}

% bold + bar/hat/tilde
% \newcommand{\alphavecbar}{\bar{\val}}
% \newcommand{\alphab}{\boldsymbol{\alpha}}
% \newcommand{\betab}{\boldsymbol{\beta}}
% \newcommand{\gammab}{\boldsymbol{\gamma}}
% \newcommand{\thetab}{\boldsymbol{\theta}}
% \newcommand{\mub}{\boldsymbol{\mu}}
% \newcommand{\xib}{\boldsymbol{\xi}}
% \newcommand{\Deltab}{\boldsymbol{\Delta}}
% \newcommand{\Pib}{\boldsymbol{\Pi}}
% \newcommand{\etab}{\boldsymbol{\eta}}
% \newcommand{\taub}{\boldsymbol{\tau}}
% \newcommand{\lambdab}{\boldsymbol{\lambda}}
% \newcommand{\rhob}{\boldsymbol{\rho}}

% \newcommand{\alphavechat}{\hat{\val}}
% \newcommand{\alphavectil}{\tilde{\val}}
% \newcommand{\valbar}{\bar{\val}}
% \newcommand{\valhat}{\hat{\val}}
% \newcommand{\valtil}{\tilde{\val}}
% \newcommand{\vthtil}{\tilde{\vth}}
% \newcommand{\vthhat}{\hat{\vth}}
% \newcommand{\vthbar}{\bar{\vth}}
% \newcommand{\vbetatil}{\tilde{\vbeta}}
% \newcommand{\vbetahat}{\hat{\vbeta}}
% \newcommand{\pitil}{\tilde{\pi}}
% \newcommand{\elltil}{\tilde{\ell}}
% \newcommand{\delhat}{\hat{\delta}}
% \newcommand{\phihat}{\hat{\phi}}
% \newcommand{\delbar}{\bar{\delta}}
% \newcommand{\alphahat}{\hat{\alpha}}
% \newcommand{\alphatil}{\tilde{\alpha}}
% \newcommand{\mubar}{\bar{\mu}}
% \newcommand{\thetahat}{\hat{\theta}}
% \newcommand{\thetabar}{\bar{\theta}}
% \newcommand{\betahat}{\hat{\beta}}
% \newcommand{\sigmahat}{\hat{\sigma}}
% \newcommand{\Deltahat}{\hat{\Delta}}
% \newcommand{\xibar}{\bar{\xi}}
% \newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
% \newcommand{\thetatil}{\tilde{\theta}}
% \newcommand{\sigmatil}{\tilde{\sigma}}
% \newcommand{\betatil}{\tilde{\beta}}
% \newcommand{\Thetatil}{\tilde{\Theta}}

==> figures/hgnn_framework.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,216); %set diagram left start at 0, and has height of 216


% Text Node
\draw    (96.5,123) .. controls (96.5,120.24) and (98.74,118) .. (101.5,118) -- (114.5,118) .. controls (117.26,118) and (119.5,120.24) .. (119.5,123) -- (119.5,131) .. controls (119.5,133.76) and (117.26,136) .. (114.5,136) -- (101.5,136) .. controls (98.74,136) and (96.5,133.76) .. (96.5,131) -- cycle  ;
\draw (97.5,119) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{13.28pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Data}
\end{center}

\end{minipage}};
% Text Node
\draw    (90.33,74.67) .. controls (90.33,71.91) and (92.57,69.67) .. (95.33,69.67) -- (121.33,69.67) .. controls (124.09,69.67) and (126.33,71.91) .. (126.33,74.67) -- (126.33,88.67) .. controls (126.33,91.43) and (124.09,93.67) .. (121.33,93.67) -- (95.33,93.67) .. controls (92.57,93.67) and (90.33,91.43) .. (90.33,88.67) -- cycle  ;
\draw (91.33,70.67) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{22.16pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Heuristic}\\{\scriptsize solver}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ]  (152.83,69.17) -- (196.83,69.17) -- (196.83,93.17) -- (152.83,93.17) -- cycle  ;
\draw (153.83,70.17) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.82pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Heuristic}\\{\scriptsize solution ($\displaystyle \mathbf{y}$)}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ]  (154.83,160.17) -- (198.83,160.17) -- (198.83,185.17) -- (154.83,185.17) -- cycle  ;
\draw (155.83,161.17) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.82pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize ML}\\{\scriptsize solution ($\displaystyle \hat{\mathbf{y}}$)}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ]  (153.67,116.17) -- (197.67,116.17) -- (197.67,134.17) -- (153.67,134.17) -- cycle  ;
\draw (154.67,117.17) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{28.06pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Evaluator $\displaystyle g$}
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (215.83,106) -- (237.83,106) -- (237.83,120) -- (215.83,120) -- cycle  ;
\draw (216.83,107) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {\begin{minipage}[lt]{12.66pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle g(\mathbf{y})$
\end{center}

\end{minipage}};
% Text Node
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (216.5,136) -- (238.5,136) -- (238.5,151) -- (216.5,151) -- cycle  ;
\draw (217.5,137) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {\begin{minipage}[lt]{12.66pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle g(\mathbf{\hat{y}})$
\end{center}

\end{minipage}};
% Text Node
\draw (258.33,116.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$ \begin{array}{l}
\ell =\ell _{CE}(\mathbf{y,\ \hat{y}})\\
\ \ \ \ \ \ \ +\ \eta \ell _{PI}( g(\mathbf{y}) ,\ g(\hat{\mathbf{y}}))
\end{array}$};
% Text Node
\draw    (93.83,165.5) .. controls (93.83,162.74) and (96.07,160.5) .. (98.83,160.5) -- (117.83,160.5) .. controls (120.59,160.5) and (122.83,162.74) .. (122.83,165.5) -- (122.83,179.5) .. controls (122.83,182.26) and (120.59,184.5) .. (117.83,184.5) -- (98.83,184.5) .. controls (96.07,184.5) and (93.83,182.26) .. (93.83,179.5) -- cycle  ;
\draw (94.83,161.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{17.44pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize HGNN}\\{\scriptsize solver}
\end{center}

\end{minipage}};
% Text Node
\draw (58.17,114.42) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{0.35em}{0.42em}\selectfont]  {$ \begin{array}{l}
\mathcal{G}_{1}(\mathbf{A,\ X}_{1} ')\\
\ \ \ \ \ \ \ \ \vdots \\
\mathcal{G}_{n}(\mathbf{A,\ X_{n} '}) \ 
\end{array}$};
% Connection
\draw    (108.07,118) -- (108.23,95.67) ;
\draw [shift={(108.25,93.67)}, rotate = 90.42] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (175.06,93.17) -- (175.46,114.17) ;
\draw [shift={(175.5,116.17)}, rotate = 268.91] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (176.53,160.17) -- (175.94,136.17) ;
\draw [shift={(175.89,134.17)}, rotate = 88.59] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (197.67,119.94) -- (213.89,116.08) ;
\draw [shift={(215.83,115.62)}, rotate = 166.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (197.67,132.95) -- (214.61,138.94) ;
\draw [shift={(216.5,139.61)}, rotate = 199.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (126.33,81.53) -- (150.83,81.35) ;
\draw [shift={(152.83,81.33)}, rotate = 179.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (196.83,83.62) .. controls (233.53,85.83) and (261.75,96.14) .. (281.49,114.53) ;
\draw [shift={(282.69,115.67)}, rotate = 223.99] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (198.83,172.25) .. controls (230.96,174.16) and (258.47,164.73) .. (281.34,143.95) ;
\draw [shift={(282.73,142.67)}, rotate = 136.87] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (108.07,136) -- (108.23,158.5) ;
\draw [shift={(108.25,160.5)}, rotate = 269.58] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (122.83,172.54) -- (152.83,172.61) ;
\draw [shift={(154.83,172.61)}, rotate = 180.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (237.83,115.44) -- (255.38,119.32) ;
\draw [shift={(257.33,119.75)}, rotate = 192.49] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (238.5,141.32) -- (255.37,137.98) ;
\draw [shift={(257.33,137.59)}, rotate = 168.79] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

\end{tikzpicture}
